Measurements of the branching fractions of $\Xi_{c}^{0}\to\Xi^{0}\pi^{0}$, $\Xi_{c}^{0}\to\Xi^{0}\eta$, and $\Xi_{c}^{0}\to\Xi^{0}\eta^{\prime}$ and asymmetry parameter of $\Xi_{c}^{0}\to\Xi^{0}\pi^{0}$

We present a study of $\Xi_{c}^{0}\to\Xi^{0}\pi^{0}$, $\Xi_{c}^{0}\to\Xi^{0}\eta$, and $\Xi_{c}^{0}\to\Xi^{0}\eta^{\prime}$ decays using the Belle and Belle~II data samples, which have integrated luminosities of 980~$\mathrm{fb}^{-1}$ and 426~$\mathrm{fb}^{-1}$, respectively. We measure the following relative branching fractions $${\cal B}(\Xi_{c}^{0}\to\Xi^{0}\pi^{0})/{\cal B}(\Xi_{c}^{0}\to\Xi^{-}\pi^{+}) = 0.48 \pm 0.02 ({\rm stat}) \pm 0.03 ({\rm syst}) ,$$ $${\cal B}(\Xi_{c}^{0}\to\Xi^{0}\eta)/{\cal B}(\Xi_{c}^{0}\to\Xi^{-}\pi^{+}) = 0.11 \pm 0.01 ({\rm stat}) \pm 0.01 ({\rm syst}) ,$$ $${\cal B}(\Xi_{c}^{0}\to\Xi^{0}\eta^{\prime})/{\cal B}(\Xi_{c}^{0}\to\Xi^{-}\pi^{+}) = 0.08 \pm 0.02 ({\rm stat}) \pm 0.01 ({\rm syst}) $$ for the first time, where the uncertainties are statistical ($\rm stat$) and systematic ($\rm syst$). By multiplying by the branching fraction of the normalization mode, ${\mathcal B}(\Xi_{c}^{0}\to\Xi^{-}\pi^{+})$, we obtain the following absolute branching fraction results $(6.9 \pm 0.3 ({\rm stat}) \pm 0.5 ({\rm syst}) \pm 1.3 ({\rm norm})) \times 10^{-3}$, $(1.6 \pm 0.2 ({\rm stat}) \pm 0.2 ({\rm syst}) \pm 0.3 ({\rm norm})) \times 10^{-3}$, and $(1.2 \pm 0.3 ({\rm stat}) \pm 0.1 ({\rm syst}) \pm 0.2 ({\rm norm})) \times 10^{-3}$, for $\Xi_{c}^{0}$ decays to $\Xi^{0}\pi^{0}$, $\Xi^{0}\eta$, and $\Xi^{0}\eta^{\prime}$ final states, respectively. The third errors are from the uncertainty on ${\mathcal B}(\Xi_{c}^{0}\to\Xi^{-}\pi^{+})$. The asymmetry parameter for $\Xi_{c}^{0}\to\Xi^{0}\pi^{0}$ is measured to be $\alpha(\Xi_{c}^{0}\to\Xi^{0}\pi^{0}) = -0.90\pm0.15({\rm stat})\pm0.23({\rm syst})$.

==> orcid.tex <==
%%% Paper:    Omega_c0 two-body decays
%%% Journal:  JHEP
%%% Contacts: X. Han, S. Jia. L. Yuan, C.P. Shen
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{pubxxx-orcid} to insert this material into your latex file.
%%% Special instructions for JHEP:
%%%  1) add ",\hbox{$\dagger$}" inside the affiliation [...] and
%%%         "\note[$\dagger$]{Corresponding author.} after the corresponding author's name.
%%%  2) add  \emailAdd{...}" for the corresponding author at the end of this file.



\collaboration{The Belle Collaboration}
  \author{X.~Han\,\orcidlink{0000-0003-1656-9413},} % 2589
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545},} % 2457
  \author{L.~Yuan\,\orcidlink{0000-0002-6719-5397},} % 14003
  \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618},} % 2464
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173},} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876},} % 2239
  \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243},} % 7423
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964},} % 2223
% \author{S.~Al~Said\,\orcidlink{0000-0002-4895-3869},} % 6823
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790},} % 4684
% \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X},} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406},} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055},} % 3747
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290},} % 3766
% \author{T.~Aziz\,\orcidlink{-},} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912},} % 5623
  \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332},} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854},} % 2115
% \author{Y.~Ban\,\orcidlink{-},} % 3503
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409},} % 8603
% \author{E.~Barberio\,\orcidlink{-},} % -229
% \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X},} % 2180
% \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387},} % 9863
  \author{P.~Behera\,\orcidlink{0000-0002-1527-2266},} % 4204
  \author{K.~Belous\,\orcidlink{0000-0003-0014-2589},} % 2329
  \author{J.~Bennett\,\orcidlink{0000-0002-5440-2668},} % 2454
% \author{F.~Bernlochner\,\orcidlink{0000-0001-8153-2719},} % 2282
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439},} % 3783
% \author{D.~Besson\,\orcidlink{-},} % 3585
  \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621},} % 2228
% \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594},} % 2097
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986},} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260},} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471},} % 8703
% \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386},} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787},} % 9643
% \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338},} % 4643
% \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918},} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913},} % 7083
% \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319},} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524},} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673},} % 2577
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007},} % 2560
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131},} % 2171
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134},} % 5223
% \author{L.~Cao\,\orcidlink{0000-0001-8332-5668},} % 2099
  \author{D.~\v{C}ervenkov\,\orcidlink{0000-0002-1865-741X},} % 2078
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058},} % 2827
  \author{P.~Chang\,\orcidlink{0000-0003-4064-388X},} % 2542
% \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288},} % 2167
  \author{A.~Chen\,\orcidlink{0000-0002-8544-9274},} % -284
% \author{C.~Chen\,\orcidlink{0000-0003-1589-9955},} % 12803
% \author{Y.~Chen\,\orcidlink{0000-0002-2057-1076},} % 2576
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850},} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429},} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053},} % 2308
  \author{H.~E.~Cho\,\orcidlink{0000-0002-7008-3759},} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399},} % 2516
% \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664},} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277},} % 2364
  \author{Y.~Choi\,\orcidlink{0000-0003-3499-7948},} % -405
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216},} % 2206
  \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585},} % 2092
% \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X},} % 12604
% \author{S.~Cunliffe\,\orcidlink{0000-0003-0167-8641},} % 2272
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373},} % 2254
% \author{S.~Das\,\orcidlink{0000-0001-6857-966X},} % 9163
% \author{N.~Dash\,\orcidlink{0000-0003-2172-3534},} % 2601
% \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793},} % 8364
  \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675},} % 2459
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X},} % 2528
  \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163},} % 9465
  \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936},} % 2065
% \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121},} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675},} % 2319
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939},} % 2215
% \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582},} % 2574
% \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970},} % 11063
% \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868},} % 5563
  \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693},} % 2551
% \author{M.~Feindt\,\orcidlink{-},} % -532
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427},} % 2482
  \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234},} % 2073
% \author{A.~Frey\,\orcidlink{0000-0001-7470-3874},} % 2150
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739},} % 2563
% \author{R.~Garg\,\orcidlink{0000-0002-7406-4707},} % 2213
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134},} % 2413
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857},} % 2510
% \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405},} % 2161
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128},} % 2106
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X},} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616},} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833},} % 2727
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652},} % 2342
% \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399},} % 2686
  \author{T.~Gu\,\orcidlink{0000-0002-1470-6536},} % 14283
% \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278},} % 2514
  \author{C.~Hadjivasiliou\,\orcidlink{0000-0002-2234-0001},} % 9503
% \author{S.~Halder\,\orcidlink{0000-0002-6280-494X},} % 4743
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871},} % 2462
  \author{T.~Hara\,\orcidlink{0000-0002-4321-0417},} % 2523
% \author{O.~Hartbrich\,\orcidlink{0000-0001-7741-4381},} % 2158
  \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X},} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903},} % 2455
% \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593},} % 7663
% \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872},} % 2265
% \author{D.~Herrmann\,\orcidlink{0000-0001-9772-9989},} % -565
% \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587},} % 2466
% \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505},} % 2485
  \author{W.-S.~Hou\,\orcidlink{0000-0002-4260-5118},} % -288
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X},} % 2299
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406},} % 2389
  \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X},} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072},} % 2323
% \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279},} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366},} % 12223
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633},} % 2281
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266},} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559},} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557},} % 2229
% \author{S.~Iwata\,\orcidlink{-},} % 4323
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336},} % 2322
  \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887},} % 6744
% \author{H.~B.~Jeon\,\orcidlink{0000-0002-0857-0353},} % 2170
  \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565},} % 16243
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830},} % 2105
% \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087},} % 4224
% \author{J.~Kahn\,\orcidlink{0000-0002-8517-2359},} % 2448
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055},} % 2391
% \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222},} % 2220
  \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X},} % 7344
% \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751},} % 2283
% \author{S.~Kang\,\orcidlink{0000-0002-5320-7043},} % 12683
% \author{P.~Kapusta\,\orcidlink{0000-0003-1235-1935},} % 6663
% \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716},} % 2550
% \author{Y.~Kato\,\orcidlink{0000-0001-6314-4288},} % 2549
% \author{H.~Kawai\,\orcidlink{-},} % 4344
% \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238},} % 4363
% \author{H.~Kichimi\,\orcidlink{0000-0003-0534-4710},} % 2233
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X},} % 2168
  \author{C.~H.~Kim\,\orcidlink{0000-0002-5743-7698},} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070},} % 2315
% \author{H.~J.~Kim\,\orcidlink{0000-0001-9787-4684},} % 4863
% \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112},} % 2118
% \author{K.~T.~Kim\,\orcidlink{0000-0003-2884-6772},} % 2409
% \author{S.~K.~Kim\,\orcidlink{-},} % 3823
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634},} % 2403
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103},} % 2379
% \author{T.~D.~Kimmel\,\orcidlink{0000-0002-9743-8249},} % 2241
% \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591},} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182},} % 2318
% \author{C.~Kleinwort\,\orcidlink{0000-0002-9017-9504},} % 2499
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349},} % 2407
% \author{I.~Komarov\,\orcidlink{0000-0001-6282-1881},} % 2210
  \author{T.~Konno\,\orcidlink{0000-0003-2487-8080},} % 2490
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172},} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968},} % 2475
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931},} % 3884
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675},} % 2474
% \author{R.~Kroeger\,\orcidlink{-},} % 2242
% \author{J.-F.~Krohn\,\orcidlink{0000-0002-5001-0675},} % 2502
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667},} % 2575
  \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049},} % 2486
  \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708},} % 2744
  \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626},} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365},} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538},} % 4083
% \author{E.~Kurihara\,\orcidlink{-},} % -95
% \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044},} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648},} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691},} % 2231
% \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421},} % 2066
% \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X},} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806},} % 2729
% \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474},} % 2277
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013},} % 10223
% \author{I.~S.~Lee\,\orcidlink{0000-0002-7786-323X},} % 2422
% \author{J.~K.~Lee\,\orcidlink{0000-0001-6397-0723},} % 2190
  \author{S.~C.~Lee\,\orcidlink{0000-0002-9835-1006},} % 2544
% \author{D.~Levit\,\orcidlink{0000-0001-5789-6205},} % 2507
% \author{P.~Lewis\,\orcidlink{0000-0002-5991-622X},} % 2582
  \author{C.~H.~Li\,\orcidlink{0000-0002-3240-4523},} % 2325
  \author{J.~Li\,\orcidlink{0000-0001-5520-5394},} % 11064
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307},} % 3263
  \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495},} % 2377
  \author{Y.~Li\,\orcidlink{0000-0002-4413-6247},} % 8083
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851},} % 2573
  \author{L.~Li~Gioi\,\orcidlink{0000-0003-2024-5649},} % 2495
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247},} % 2262
  \author{K.~Lieret\,\orcidlink{0000-0003-2792-7511},} % 2268
% \author{Y.-R.~Lin\,\orcidlink{0000-0003-0864-6693},} % 9323
% \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131},} % 3565
% \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056},} % 2578
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784},} % 3268
% \author{J.~MacNaughton\,\orcidlink{-},} % -550
% \author{A.~Martini\,\orcidlink{0000-0003-1161-4983},} % 2336
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583},} % 2238
% \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X},} % 5543
% \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448},} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777},} % 9763
% \author{F.~Meier\,\orcidlink{0000-0002-6088-0412},} % 3103
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108},} % 2456
% \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X},} % 2296
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X},} % 2327
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236},} % 2452
% \author{H.~Miyata\,\orcidlink{0000-0002-1026-2894},} % 2071
  \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969},} % 2483
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666},} % 2278
% \author{H.~K.~Moon\,\orcidlink{0000-0001-5213-6477},} % 2304
% \author{T.~J.~Moon\,\orcidlink{0000-0001-9886-8534},} % 2397
% \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951},} % 2120
% \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005},} % 2527
% \author{T.~M\"uller\,\orcidlink{0000-0003-4337-0098},} % 2165
  \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071},} % 2372
  \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456},} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355},} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217},} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328},} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075},} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967},} % 2232
  \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628},} % 2335
% \author{D.~Narwal\,\orcidlink{0000-0001-6585-7767},} % 7223
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291},} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X},} % 12063
% \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X},} % 9464
% \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692},} % 2371
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741},} % 2477
% \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X},} % 2063
  \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253},} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346},} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922},} % 3063
% \author{K.~Ogawa\,\orcidlink{0000-0003-2220-7224},} % 2430
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079},} % 6263
% \author{S.~Okuno\,\orcidlink{-},} % -164
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885},} % 4563
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064},} % 2160
  \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847},} % 2331
% \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936},} % 9623
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881},} % 2984
% \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824},} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022},} % 2188
% \author{T.~Pang\,\orcidlink{0000-0003-1204-0846},} % 2114
% \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537},} % 2532
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052},} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028},} % 18203
% \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218},} % 2509
% \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411},} % 2116
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091},} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437},} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373},} % 2421
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470},} % 2476
% \author{F.~Pham\,\orcidlink{0000-0003-0608-2302},} % 2963
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748},} % 2346
% \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X},} % 11223
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583},} % 2096
% \author{S.~Prell\,\orcidlink{0000-0002-0195-8005},} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493},} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450},} % 2501
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689},} % 2196
% \author{A.~Rabusov\,\orcidlink{0000-0001-8189-7398},} % 2355
% \author{M.~Ritter\,\orcidlink{0000-0001-6507-4631},} % 2580
% \author{M.~R\"{o}hrken\,\orcidlink{0000-0003-0654-2866},} % 11883
% \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152},} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638},} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021},} % 2205
  \author{G.~Russo\,\orcidlink{0000-0001-5823-4393},} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413},} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409},} % 2175
% \author{M.~Salehi\,\orcidlink{-},} % 2127
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369},} % 2286
% \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X},} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956},} % 2185
% \author{T.~Sanuki\,\orcidlink{0000-0002-4537-5899},} % 6783
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830},} % 2292
% \author{P.~Schmolz\,\orcidlink{-},} % 4685
% \author{O.~Schneider\,\orcidlink{-},} % -198
  \author{G.~Schnell\,\orcidlink{0000-0002-7336-3246},} % 12204
  \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953},} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028},} % 2108
% \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983},} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732},} % 2405
% \author{R.~Seidl\,\orcidlink{0000-0002-6552-6973},} % -115
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255},} % 2517
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118},} % 2987
% \author{O.~Seon\,\orcidlink{-},} % 2581
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X},} % 2328
  \author{W.~Shan\,\orcidlink{0000-0003-2811-2218},} % 11943
  \author{M.~Shapkin\,\orcidlink{0000-0002-4098-9592},} % 2460
  \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429},} % 11584
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957},} % 2339
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270},} % 2234
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639},} % 2412
  \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496},} % 2122
% \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895},} % 2419
% \author{F.~Simon\,\orcidlink{0000-0002-5978-0289},} % 2164
% \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462},} % 2903
% \author{R.~Sinha\,\orcidlink{-},} % 3423
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474},} % 2243
% \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091},} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827},} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059},} % 2398
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381},} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944},} % 2326
% \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333},} % 2267
% \author{J.~F.~Strube\,\orcidlink{0000-0001-7470-9301},} % 2451
% \author{J.~Stypula\,\orcidlink{0000-0002-5844-7476},} % 2368
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585},} % 4243
% \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210},} % 2583
  \author{T.~Sumiyoshi\,\orcidlink{0000-0002-0486-3896},} % 4184
% \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582},} % 3784
% \author{S.~Y.~Suzuki\,\orcidlink{0000-0002-7135-4901},} % 2496
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973},} % 2437
% \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706},} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216},} % 2530
% \author{S.~S.~Tang\,\orcidlink{0000-0001-6564-0445},} % 12003
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746},} % 3803
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564},} % 2285
% \author{Y.~Tao\,\orcidlink{0000-0002-9186-2591},} % 2362
% \author{G.~N.~Taylor\,\orcidlink{-},} % -220
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377},} % 2546
% \author{Y.~Teramoto\,\orcidlink{-},} % -349
% \author{A.~Thampi\,\orcidlink{-},} % 7403
% \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883},} % 10403
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036},} % 2369
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997},} % 2361
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168},} % 2370
% \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344},} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016},} % 2586
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830},} % 2252
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X},} % 2420
  \author{K.~Uno\,\orcidlink{0000-0002-2209-8198},} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480},} % 2149
  \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953},} % 2302
% \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X},} % 2317
% \author{Y.~Usov\,\orcidlink{0000-0003-3144-2920},} % 5003
  \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824},} % 2251
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816},} % 2706
  \author{G.~Varner\,\orcidlink{0000-0002-0302-8151},} % 2119
% \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295},} % 2545
  \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056},} % 2289
% \author{V.~Vorobyev\,\orcidlink{0000-0002-6660-868X},} % 2298
% \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936},} % 2249
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363},} % 2226
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952},} % 2569
% \author{C.~H.~Wang\,\orcidlink{0000-0001-6760-9839},} % 2224
% \author{D.~Wang\,\orcidlink{0000-0003-1485-2143},} % 10003
% \author{E.~Wang\,\orcidlink{0000-0001-6391-5118},} % 10983
% \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341},} % 2074
  \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255},} % 2076
% \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694},} % 2309
% \author{Y.~Watanabe\,\orcidlink{-},} % -165
% \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628},} % 6843
% \author{S.~Wehle\,\orcidlink{0000-0002-6168-1829},} % 2489
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773},} % 6123
% \author{E.~Widmann\,\orcidlink{-},} % -509
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072},} % 2604
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442},} % 2410
% \author{X.~Xu\,\orcidlink{0000-0001-5096-1182},} % 4923
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474},} % 3645
% \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336},} % 2492
% \author{H.~Yamamoto\,\orcidlink{-},} % 2964
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871},} % 2094
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971},} % 2374
% \author{H.~Ye\,\orcidlink{0000-0003-0552-5490},} % 2537
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346},} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349},} % 2365
% \author{Y.~Yook\,\orcidlink{0000-0002-4912-048X},} % 2453
  \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686},} % 2088
% \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748},} % 2357
% \author{Y.~Zhai\,\orcidlink{0000-0001-7207-5122},} % 12703
% \author{J.~Zhang\,\orcidlink{0000-0001-6535-0659},} % 2349
  \author{Z.~P.~Zhang\,\orcidlink{0000-0001-6140-2044},} % 5363
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565},} % 4703
  \author{V.~Zhukova\,\orcidlink{0000-0002-8253-641X},} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983


==> pub052.tex <==
%%% Paper:    Xi_c0 decays
%%% Journal:  JHEP
%%% Contacts: J.X. Cui, S. Jia, C.P. Shen
%%% ====================================================================
%%% Use \input{pub052} to insert this material into your latex file.
\newcounter{AffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCPPM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYerevan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGoettingen{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instBeihang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBINP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instCMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCinvestavIPN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPrague{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChiangMai{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChiba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChonnam{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChula{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instConacyt{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDESY{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDuke{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instITAR{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFuJen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFudan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGifu{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSOKENDAI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMainz{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGyeongsang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHanyang{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHeidelberg{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKEK{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJPARC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHiroshima{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHUNNU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIKERBASQUE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFrascati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISc{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIISER{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITBhubaneswar{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITGuwahati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITHyderabad{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIITJodhpur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITMadras{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIndiana{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIHEPRussia{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHEPHYVienna{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPChina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIOP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIFIC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instISU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJAEA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJLU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKarlsruhe{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKitasato{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKISTI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKoreaUnivKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyotoU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyungpook{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instLNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGiessen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLuther{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMNITJaipur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMcGill{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMETU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMEPhI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoyaKMI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNankai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNaraWu{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUNAM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHSE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNTUTaiwan{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNUUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKrakow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNiigata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOsakaMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRCNP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPNNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMPGHLL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjabPAU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instRIKENBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRIKENMSL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSeoul{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instShandong{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyiv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSPU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoochow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoongsil{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSEU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaJSI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSKKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTelAviv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instToho{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTohoku{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTitech{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTokyoMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUAS{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIJCLab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPHC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instAdelaide{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUofA{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instBilbao{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBonn{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUBC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCincinnati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFlorida{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHamburg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHawaii{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUniLJ{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLouisville{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMalaya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instManitoba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMelbourne{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMississippi{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUOM{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNovaGorica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUPES{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPittsburgh{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUSTC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSAlabama{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSCarolina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSydney{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTabuk{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUTokyo{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instEri{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVictoria{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUppsala{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVPI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instWayneState{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instXavier{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXJTU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYamagata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYonsei{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTYL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instZZU{\protect\theAffiliationCounter}
\collaboration{The Belle and Belle II Collaborations}
  \author[\instKEK,\instSOKENDAI]{I.~Adachi,} % 2590
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{K.~Adamczyk,} % 2239
  \author[\instPanjab]{L.~Aggarwal,} % 10083
% \author[\instBonn]{P.~Ahlburg,} % 2367
% \author[\instXavier]{H.~Ahmed,} % 11323
% \author[\instKoreaUnivKU]{J.~K.~Ahn,} % 7423
  \author[\instUTokyo]{H.~Aihara,} % 2223
  \author[\instYerevan]{N.~Akopov,} % 9443
  \author[\instNapoliUNIV,\instNapoliINFN]{A.~Aloisio,} % 2194
% \author[\instTabuk,\instKAU]{S.~Al~Said,} % 6823
  \author[\instTabuk]{N.~Althubiti,} % 21524
% \author[\instMPGHLL]{L.~Andricek,} % 2098
% \author[\instBonn]{M.~Angelsmark,} % 13963
  \author[\instIOP]{N.~Anh~Ky,} % 2218
  \author[\instBNL]{D.~M.~Asner,} % 4684
  \author[\instCincinnati]{H.~Atmacan,} % 2538
% \author[\instBINP,\instNSU]{V.~Aulchenko,} % 8183
  \author[\instHSE]{T.~Aushev,} % 3747
  \author[\instKyiv]{V.~Aushev,} % 2155
  \author[\instNagoya]{M.~Aversano,} % 7363
  \author[\instTabuk]{R.~Ayad,} % 3766
% \author[\instTata]{T.~Aziz,} % 3523
  \author[\instIPHC]{V.~Babu,} % 5623
% \author[\instKrakow]{S.~Bacher,} % 2258
  \author[\instKEK]{H.~Bae,} % 10863
  \author[\instIITBhubaneswar]{S.~Bahinipati,} % 2332
% \author[\instSydney]{A.~M.~Bakich,} % 2115
  \author[\instIJCLab]{P.~Bambade,} % 3003
  \author[\instLouisville]{Sw.~Banerjee,} % 8603
% \author[\instPanjab]{S.~Bansal,} % 5163
  \author[\instKEK]{M.~Barrett,} % 2180
% \author[\instPisaUNIV,\instPisaINFN]{G.~Batignani,} % 6643
  \author[\instIPHC]{J.~Baudot,} % 2562
% \author[\instKarlsruhe]{M.~Bauer,} % 9863
  \author[\instDESY]{A.~Baur,} % 5683
  \author[\instVictoria]{A.~Beaubien,} % 6683
  \author[\instDESY]{F.~Becherer,} % 21623
  \author[\instKarlsruhe]{J.~Becker,} % 5403
% \author[\instIITMadras]{P.~K.~Behera,} % 4204
% \author[\instIHEPRussia]{K.~Belous,} % 2329
  \author[\instMississippi]{J.~V.~Bennett,} % 2454
% \author[\instRomaTreINFN]{E.~Bernieri,} % 4483
  \author[\instBonn]{F.~U.~Bernlochner,} % 2282
  \author[\instCPPM]{V.~Bertacchi,} % 2212
  \author[\instHEPHYVienna]{M.~Bertemes,} % 2595
  \author[\instTelAviv]{E.~Bertholet,} % 13163
  \author[\instHawaii]{M.~Bessner,} % 3783
% \author[\instMEPhI]{D.~Besson,} % 3585
  \author[\instPisaUNIV,\instPisaINFN]{S.~Bettarini,} % 2350
% \author[\instIISER]{V.~Bhardwaj,} % 2228
  \author[\instIITGuwahati]{B.~Bhuyan,} % 2097
  \author[\instTorinoUNIV,\instTorinoINFN]{F.~Bianchi,} % 2564
  \author[\instTUM]{L.~Bierwirth,} % 11723
  \author[\instDESY]{T.~Bilka,} % 2484
% \author[\instLMU]{S.~Bilokin,} % 3623
  \author[\instLouisville]{D.~Biswas,} % 8703
% \author[\instKEK]{T.~Bloomfield,} % 2418
  \author[\instBINP,\instNSU]{A.~Bobrov,} % 2294
  \author[\instSoochow,\instHSE]{D.~Bodrov,} % 9643
% \author[\instDESY]{A.~Bolz,} % 15403
% \author[\instBINP,\instNSU]{A.~Bondar,} % 4643
% \author[\instWayneState]{G.~Bonvicini,} % 2095
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{J.~Borah,} % 7083
  \author[\instTorinoUNIV,\instTorinoINFN]{A.~Boschetti,} % 17683
  \author[\instKrakow]{A.~Bozek,} % 2303
  \author[\instLjubljanaJSI,\instLjubljanaUM]{M.~Bra\v{c}ko,} % 2425
  \author[\instRomaTreINFN]{P.~Branchini,} % 2577
% \author[\instISU]{N.~Brenny,} % 19943
% \author[\instCMU]{R.~A.~Briere,} % 2584
  \author[\instHawaii]{T.~E.~Browder,} % 2560
% \author[\instGoettingen]{Y.~Buch,} % 17323
  \author[\instRomaTreINFN]{A.~Budano,} % 2171
  \author[\instRomaTreUNIV,\instRomaTreINFN]{S.~Bussino,} % 5384
% \author[\instFrascati]{A.~Calcaterra,} % 19163
  \author[\instMississippi]{Q.~Campagna,} % 21563
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Campajola,} % 5223
  \author[\instDESY]{L.~Cao,} % 2099
  \author[\instPisaUNIV,\instPisaINFN]{G.~Casarosa,} % 2491
  \author[\instPerugiaUNIV,\instPerugiaINFN]{C.~Cecchi,} % 2433
  \author[\instIPHC]{J.~Cerasoli,} % 20746
  \author[\instFuJen]{M.-C.~Chang,} % 2827
  \author[\instNTUTaiwan]{P.~Chang,} % 2542
% \author[\instDESY]{R.~Cheaib,} % 2208
  \author[\instSydney]{P.~Cheema,} % 15264
% \author[\instMPP]{V.~Chekelian,} % 2167
  \author[\instISU]{C.~Chen,} % 12803
% \author[\instJLU]{Y.~Q.~Chen,} % 16264
% \author[\instNTUTaiwan]{Y.-T.~Chen,} % 2884
  \author[\instHanyang]{B.~G.~Cheon,} % 2173
  \author[\instBINP]{K.~Chilikin,} % 2308
  \author[\instChiangMai]{K.~Chirapatpimol,} % 10803
  \author[\instHanyang]{H.-E.~Cho,} % 2182
  \author[\instKISTI]{K.~Cho,} % 2516
  \author[\instYonsei]{S.-J.~Cho,} % 2723
  \author[\instCAU]{S.-K.~Choi,} % 2364
  \author[\instISU]{S.~Choudhury,} % 2206
% \author[\instWayneState]{D.~Cinabro,} % 2092
% \author[\instISU]{J.~Cochran,} % 12604
  \author[\instPisaUNIV,\instPisaINFN]{L.~Corona,} % 3944
% \author[\instMississippi]{L.~M.~Cremaldi,} % 2276
  \author[\instSEU]{J.~X.~Cui,} % 8863
% \author[\instTokyoMetropolitan]{T.~Czank,} % 2254
% \author[\instMNITJaipur]{S.~Das,} % 9163
  \author[\instDESY]{F.~Dattola,} % 3745
  \author[\instCinvestavIPN]{E.~De~La~Cruz-Burelo,} % 2359
  \author[\instAdelaide]{S.~A.~De~La~Motte,} % 2128
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{G.~de~Marino,} % 8364
  \author[\instNapoliUNIV,\instNapoliINFN]{G.~De~Nardo,} % 2459
% \author[\instUBC]{M.~De~Nuccio,} % 2610
  \author[\instKarlsruhe]{G.~De~Pietro,} % 2528
  \author[\instFrascati]{R.~de~Sangro,} % 2524
% \author[\instBonn]{B.~Deschamps,} % 2671
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Destefanis,} % 2594
  \author[\instKEK]{S.~Dey,} % 5023
% \author[\instCinvestavIPN]{A.~De~Yta-Hernandez,} % 2104
  \author[\instIITHyderabad]{R.~Dhamija,} % 9465
  \author[\instBNL]{A.~Di~Canto,} % 10963
  \author[\instNapoliUNIV,\instNapoliINFN]{F.~Di~Capua,} % 2065
  \author[\instBonn]{J.~Dingfelder,} % 2151
  \author[\instPrague]{Z.~Dole\v{z}al,} % 2319
  \author[\instUAS]{I.~Dom\'{\i}nguez~Jim\'{e}nez,} % 2191
  \author[\instITAR]{T.~V.~Dong,} % 2215
  \author[\instTriesteINFN]{M.~Dorigo,} % 12543
% \author[\instHEPHYVienna]{D.~Dorner,} % 13564
  \author[\instGiessen]{K.~Dort,} % 5583
  \author[\instMelbourne]{D.~Dossett,} % 2574
% \author[\instDESY]{S.~Dreyer,} % 12823
  \author[\instHawaii]{S.~Dubey,} % 11063
% \author[\instBonn]{S.~Duell,} % 2344
  \author[\instTUM]{K.~Dugic,} % 11103
  \author[\instIPHC]{G.~Dujany,} % 9703
  \author[\instKarlsruhe]{P.~Ecker,} % 5563
  \author[\instBonn]{M.~Eliachevitch,} % 2725
  \author[\instBINP,\instNSU]{D.~Epifanov,} % 2551
% \author[\instDESY]{Y.~Fan,} % 21303
  \author[\instHEPHYVienna]{P.~Feichtinger,} % 9843
  \author[\instKarlsruhe]{T.~Ferber,} % 2482
% \author[\instMelbourne]{D.~Ferlewicz,} % 2073
  \author[\instKEK]{T.~Fillinger,} % 9803
  \author[\instIPHC]{C.~Finck,} % 15803
% \author[\instFrascati]{G.~Finocchiaro,} % 2400
% \author[\instHeidelberg]{P.~Fischer,} % 2141
% \author[\instHawaii]{K.~Flood,} % 12103
  \author[\instMcGill]{A.~Fodor,} % 2312
  \author[\instPisaUNIV,\instPisaINFN]{F.~Forti,} % 2432
  \author[\instGoettingen]{A.~Frey,} % 2150
% \author[\instHEPHYVienna]{M.~Friedl,} % 2442
  \author[\instPNNL]{B.~G.~Fulsom,} % 2563
  \author[\instTriesteUNIV,\instTriesteINFN]{A.~Gabrielli,} % 13523
% \author[\instBINP,\instNSU]{N.~Gabyshev,} % 2510
% \author[\instDESY]{E.~Ganiev,} % 4623
% \author[\instKEK]{M.~Garcia-Hernandez,} % 4823
% \author[\instCMU]{R.~Garg,} % 2213
% \author[\instBINP,\instNSU]{A.~Garmash,} % 2161
  \author[\instNapoliINFN]{G.~Gaudino,} % 16563
  \author[\instUPES]{V.~Gaur,} % 2413
  \author[\instPadovaUNIV,\instPadovaINFN]{A.~Gaz,} % 2181
% \author[\instGoettingen]{U.~Gebauer,} % 2174
  \author[\instDESY]{A.~Gellrich,} % 2480
  \author[\instYerevan]{G.~Ghevondyan,} % 9445
  \author[\instTriesteUNIV,\instTriesteINFN]{D.~Ghosh,} % 11923
  \author[\instYerevan]{H.~Ghumaryan,} % 19543
  \author[\instBonn]{G.~Giakoustidis,} % 13723
  \author[\instNapoliUNIV,\instNapoliINFN]{R.~Giordano,} % 2103
  \author[\instIITHyderabad]{A.~Giri,} % 2106
  \author[\instDESY]{A.~Glazov,} % 2473
  \author[\instTriesteINFN]{B.~Gobbo,} % 2109
  \author[\instSAlabama]{R.~Godang,} % 2449
  \author[\instKyiv]{O.~Gogota,} % 2334
  \author[\instKarlsruhe]{P.~Goldenzweig,} % 2345
% \author[\instLjubljanaUniLJ,\instNovaGorica,\instLjubljanaJSI]{B.~Golob,} % 3703
% \author[\instUSTC]{G.~Gong,} % 2727
% \author[\instAdelaide]{P.~Grace,} % 9563
  \author[\instMainz]{W.~Gradl,} % 2570
% \author[\instDESY]{M.~Graf-Schreiber,} % 2730
% \author[\instVictoria]{T.~Grammatico,} % 20623
% \author[\instBonn]{S.~Granderath,} % 8383
  \author[\instRomaTreINFN]{E.~Graziani,} % 2342
  \author[\instTUM]{D.~Greenwald,} % 2686
  \author[\instPrague]{Z.~Gruberov\'{a},} % 8824
  \author[\instPittsburgh]{T.~Gu,} % 14283
% \author[\instCincinnati]{Y.~Guan,} % 2514
  \author[\instBINP,\instNSU]{K.~Gudkova,} % 10504
  \author[\instKarlsruhe]{I.~Haide,} % 14824
% \author[\instHEPHYVienna]{H.~Haigh,} % 16744
  \author[\instTata]{S.~Halder,} % 4743
  \author[\instDESY]{Y.~Han,} % 19663
% \author[\instKEK,\instSOKENDAI]{K.~Hara,} % 2462
  \author[\instKEK,\instSOKENDAI]{T.~Hara,} % 2523
  \author[\instAdelaide]{C.~Harris,} % 21383
% \author[\instHawaii]{O.~Hartbrich,} % 2158
  \author[\instNiigata]{K.~Hayasaka,} % 2330
  \author[\instNaraWu]{H.~Hayashii,} % 2455
  \author[\instMPP]{S.~Hazra,} % 7663
  \author[\instUBC,\instIPP]{C.~Hearty,} % 2450
  \author[\instBonn]{M.~T.~Hedges,} % 2265
  \author[\instKarlsruhe]{A.~Heidelbach,} % 16923
  \author[\instCinvestavIPN,\instConacyt]{I.~Heredia~de~la~Cruz,} % 2559
% \author[\instBNL,\instDESY]{M.~Hern\'{a}ndez~Villanueva,} % 2466
% \author[\instUBC]{A.~Hershenhorn,} % 2552
  \author[\instIPMU]{T.~Higuchi,} % 2485
% \author[\instNagoya]{H.~Hirata,} % 2070
  \author[\instMainz]{M.~Hoek,} % 2101
  \author[\instMelbourne]{M.~Hohmann,} % 2077
  \author[\instHEPHYVienna]{P.~Horak,} % 13583
% \author[\instRCNP]{T.~Hotta,} % 2084
  \author[\instSydney]{C.-L.~Hsu,} % 2299
% \author[\instNTUTaiwan]{K.~Huang,} % 2389
  \author[\instDESY]{T.~Humair,} % 10643
% \author[\instNagoya,\instNagoyaKMI,\instKEK]{T.~Iijima,} % 2446
  \author[\instNagoya,\instKEK]{K.~Inami,} % 2323
% \author[\instHEPHYVienna]{G.~Inguglia,} % 2500
  \author[\instIITHyderabad]{N.~Ipsita,} % 12223
% \author[\instKarlsruhe]{J.~Irakkathil~Jabbar,} % 7343
  \author[\instKEK,\instSOKENDAI]{A.~Ishikawa,} % 2281
% \author[\instKEK]{S.~Ito,} % 17463
  \author[\instKEK,\instSOKENDAI]{R.~Itoh,} % 2487
  \author[\instOsakaMetropolitan]{M.~Iwasaki,} % 2360
% \author[\instKEK]{Y.~Iwasaki,} % 2229
% \author[\instTokyoMetropolitan]{S.~Iwata,} % 4323
% \author[\instAdelaide]{P.~Jackson,} % 2255
  \author[\instIndiana]{W.~W.~Jacobs,} % 2322
% \author[\instBNL]{D.~E.~Jaffe,} % 3663
  \author[\instGyeongsang]{E.-J.~Jang,} % 6744
% \author[\instHNU]{Q.~P.~Ji,} % 16243
  \author[\instSEU]{S.~Jia,} % 2457
  \author[\instBNL]{Y.~Jin,} % 2105
  \author[\instIITMadras]{A.~Johnson,} % 16143
  \author[\instChonnam]{K.~K.~Joo,} % 4224
  \author[\instBonn]{H.~Junkerkalefeld,} % 12963
% \author[\instKyiv]{I.~Kadenko,} % 3843
% \author[\instTokyoMetropolitan]{H.~Kakuno,} % 2391
  \author[\instKrakow]{M.~Kaleta,} % 5603
% \author[\instIITGuwahati]{D.~Kalita,} % 2220
% \author[\instHEPHYVienna]{A.~B.~Kaliyar,} % 7344
  \author[\instPadovaINFN]{J.~Kandra,} % 2541
  \author[\instIPMU]{K.~H.~Kang,} % 2283
  \author[\instISU]{S.~Kang,} % 12683
% \author[\instKrakow]{P.~Kapusta,} % 6663
  \author[\instYerevan]{G.~Karyan,} % 2550
% \author[\instNagoya,\instNagoyaKMI]{Y.~Kato,} % 2549
% \author[\instChiba]{H.~Kawai,} % 4344
% \author[\instKitasato]{T.~Kawasaki,} % 4363
  \author[\instMainz]{F.~Keil,} % 19523
% \author[\instHawaii]{C.~Ketter,} % 2236
% \author[\instBonn]{M.~Khan,} % 15644
  \author[\instMPP]{C.~Kiesling,} % 2168
  \author[\instHanyang]{C.-H.~Kim,} % 2358
  \author[\instSoongsil]{D.~Y.~Kim,} % 2315
% \author[\instKyungpook]{H.~J.~Kim,} % 4863
  \author[\instKISTI]{K.-H.~Kim,} % 2118
% \author[\instKoreaUnivKU]{K.~Kim,} % 2409
  \author[\instYonsei]{Y.-K.~Kim,} % 2379
% \author[\instKoreaUnivKU]{Y.~J.~Kim,} % 2403
  \author[\instVPI,\instKEK]{H.~Kindo,} % 2195
  \author[\instCincinnati]{K.~Kinoshita,} % 2318
% \author[\instDESY]{C.~Kleinwort,} % 2499
  \author[\instPrague]{P.~Kody\v{s},} % 2407
  \author[\instKEK]{T.~Koga,} % 6963
  \author[\instHawaii]{S.~Kohani,} % 9143
  \author[\instNagoya]{K.~Kojima,} % 6363
% \author[\instKitasato]{T.~Konno,} % 2490
% \author[\instHawaii]{H.~Korandla,} % 18783
  \author[\instBINP,\instNSU]{A.~Korobov,} % 4185
  \author[\instLjubljanaJSI,\instLjubljanaUM]{S.~Korpar,} % 2475
% \author[\instIJCLab]{E.~Kou,} % 3765
  \author[\instBINP,\instNSU]{E.~Kovalenko,} % 3884
  \author[\instVictoria]{R.~Kowalewski,} % 2293
% \author[\instMPP]{T.~M.~G.~Kraetzschmar,} % 7543
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Kri\v{z}an,} % 2474
% \author[\instMississippi]{R.~Kroeger,} % 2242
% \author[\instMelbourne]{J.~F.~Krohn,} % 2502
  \author[\instBINP,\instNSU]{P.~Krokovny,} % 2575
% \author[\instGiessen]{W.~Kuehn,} % 2534
% \author[\instDESY,\instLMU]{M.~K\"{u}nzel,} % 2139
  \author[\instLMU]{T.~Kuhr,} % 2486
  \author[\instLMU]{Y.~Kulii,} % 9823
% \author[\instIITJodhpur]{J.~Kumar,} % 6464
% \author[\instIISER]{M.~Kumar,} % 2744
  \author[\instPanjabPAU]{R.~Kumar,} % 2189
  \author[\instMississippi]{K.~Kumara,} % 2257
% \author[\instTokyoMetropolitan]{T.~Kumita,} % 4083
  \author[\instKEK]{T.~Kunigo,} % 10104
% \author[\instNaraWu]{A.~Kusudo,} % 14623
  \author[\instBINP,\instNSU]{A.~Kuzmin,} % 2520
% \author[\instPrague]{P.~Kvasni\v{c}ka,} % 2184
  \author[\instYonsei]{Y.-J.~Kwon,} % 2231
  \author[\instPadovaINFN]{S.~Lacaprara,} % 2447
% \author[\instKEK]{Y.-T.~Lai,} % 2066
  \author[\instMNITJaipur]{K.~Lalwani,} % 2142
  \author[\instVPI]{T.~Lam,} % 2729
% \author[\instTriesteINFN]{L.~Lanceri,} % 2540
  \author[\instGiessen]{J.~S.~Lange,} % 2277
  \author[\instUppsala]{M.~Laurenza,} % 10223
% \author[\instCPPM]{K.~Lautenbach,} % 2102
% \author[\instBNL]{P.~J.~Laycock,} % 7683
  \author[\instUBC]{R.~Leboucher,} % 14083
% \author[\instIJCLab]{F.~R.~Le~Diberder,} % 3267
% \author[\instSeoul]{J.~K.~Lee,} % 2190
  \author[\instSKKU]{M.~J.~Lee,} % 21803
% \author[\instKyungpook]{S.~C.~Lee,} % 2544
% \author[\instMPP]{P.~Leitl,} % 2414
  \author[\instCPPM]{C.~Lemettais,} % 22704
  \author[\instDESY,\instHamburg]{P.~Leo,} % 19823
  \author[\instKEK]{D.~Levit,} % 2507
  \author[\instHawaii]{P.~M.~Lewis,} % 2582
% \author[\instLNNU]{C.~Li,} % 2325
  \author[\instCincinnati]{L.~K.~Li,} % 3263
  \author[\instFudan]{S.~X.~Li,} % 2377
  \author[\instFudan]{Y.~Li,} % 8083
  \author[\instXJTU]{Y.~B.~Li,} % 2573
  \author[\instIITMadras]{J.~Libby,} % 2262
% \author[\instLMU]{K.~Lieret,} % 2268
% \author[\instNTUTaiwan]{J.~Lin,} % 2401
  \author[\instHiroshima]{Z.~Liptak,} % 3565
  \author[\instFudan]{M.~H.~Liu,} % 15244
  \author[\instHawaii]{Q.~Y.~Liu,} % 7045
% \author[\instKEK,\instSOKENDAI]{Y.~Liu,} % 16223
% \author[\instIHEPChina]{Z.~A.~Liu,} % 3283
  \author[\instShandong]{Z.~Q.~Liu,} % 11303
  \author[\instWayneState,\instKEK]{D.~Liventsev,} % 2578
  \author[\instManitoba]{S.~Longo,} % 2396
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Lozar,} % 12423
  \author[\instLMU]{T.~Lueck,} % 2406
% \author[\instFudan]{T.~Luo,} % 3268
  \author[\instBonn]{C.~Lyu,} % 12484
  \author[\instRIKENMSL]{Y.~Ma,} % 16883
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Maggiora,} % 5343
  \author[\instIITHyderabad]{S.~P.~Maharana,} % 19083
  \author[\instTorinoINFN]{R.~Maiti,} % 12043
  \author[\instIITBhubaneswar]{S.~Maity,} % 2985
  \author[\instCPPM]{G.~Mancinelli,} % 20743
  \author[\instBNL]{R.~Manfredi,} % 10303
  \author[\instPerugiaINFN]{E.~Manoni,} % 2305
% \author[\instBonn]{A.~C.~Manthei,} % 15023
  \author[\instTriesteUNIV,\instTriesteINFN]{M.~Mantovano,} % 19783
  \author[\instMelbourne]{D.~Marcantonio,} % 11163
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Marcello,} % 4223
  \author[\instIFIC]{C.~Marinas,} % 2133
% \author[\instIPHC]{L.~Martel,} % 13503
  \author[\instRomaTreINFN]{C.~Martellini,} % 16983
  \author[\instIJCLab]{A.~Martens,} % 13823
  \author[\instDESY]{A.~Martini,} % 2336
  \author[\instDESY]{T.~Martinov,} % 19463
  \author[\instPisaUNIV,\instPisaINFN]{L.~Massaccesi,} % 16323
  \author[\instRCNP,\instEri]{M.~Masuda,} % 2238
% \author[\instUOM]{T.~Matsuda,} % 5543
% \author[\instKEK,\instNagoya]{K.~Matsuoka,} % 2316
  \author[\instBINP,\instNSU]{D.~Matvienko,} % 2351
  \author[\instIITGuwahati]{S.~K.~Maurya,} % 9763
% \author[\instIJCLab]{F.~Mawas,} % 20943
  \author[\instUBC]{J.~A.~McKenna,} % 2392
% \author[\instMPP]{F.~Meggendorfer,} % 7103
  \author[\instTata]{R.~Mehta,} % 15203
  \author[\instDuke]{F.~Meier,} % 3103
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Merola,} % 2456
% \author[\instBonn]{F.~Metzner,} % 2296
% \author[\instMelbourne]{M.~Milesi,} % 5443
  \author[\instVictoria]{C.~Miller,} % 2273
  \author[\instNapoliINFN]{M.~Mirra,} % 14744
  \author[\instISU]{S.~Mitra,} % 19944
  \author[\instNaraWu,\instKEK]{K.~Miyabayashi,} % 2327
% \author[\instKEK,\instSOKENDAI]{H.~Miyake,} % 2452
% \author[\instIJCLab]{R.~Mizuk,} % 2483
  \author[\instTata]{G.~B.~Mohanty,} % 2278
% \author[\instCinvestavIPN]{N.~Molina-Gonzalez,} % 8004
% \author[\instPisaUNIV,\instPisaINFN]{S.~Mondal,} % 19743
  \author[\instPerugiaUNIV,\instPerugiaINFN]{S.~Moneta,} % 13303
% \author[\instKoreaUnivKU]{H.~Moon,} % 2304
  \author[\instMPP]{H.-G.~Moser,} % 2120
  \author[\instHEPHYVienna]{M.~Mrvar,} % 2527
% \author[\instKarlsruhe]{Th.~Muller,} % 2165
% \author[\instTorinoINFN]{R.~Mussa,} % 2372
  \author[\instKEK,\instSOKENDAI]{I.~Nakamura,} % 3463
% \author[\instKEK,\instSOKENDAI]{K.~R.~Nakamura,} % 2417
% \author[\instOsakaMetropolitan]{E.~Nakano,} % 2554
% \author[\instRCNP]{T.~Nakano,} % 2983
  \author[\instKEK,\instSOKENDAI]{M.~Nakao,} % 2498
% \author[\instKEK,\instSOKENDAI]{H.~Nakayama,} % 2232
% \author[\instNTUTaiwan]{H.~Nakazawa,} % 2335
  \author[\instNagoya,\instNagoyaKMI]{Y.~Nakazawa,} % 17383
% \author[\instDESY]{A.~Narimani~Charan,} % 10143
  \author[\instKyotoU]{M.~Naruki,} % 4583
% \author[\instIITGuwahati]{D.~Narwal,} % 7223
  \author[\instKrakow]{Z.~Natkaniec,} % 3923
  \author[\instBNL]{A.~Natochii,} % 12063
% \author[\instIITHyderabad]{L.~Nayak,} % 9464
  \author[\instIISc]{M.~Nayak,} % 2371
  \author[\instYerevan]{G.~Nazaryan,} % 9523
  \author[\instKarlsruhe]{M.~Neu,} % 23304
% \author[\instDESY]{C.~Niebuhr,} % 2477
  \author[\instKSU]{M.~Niiyama,} % 2063
% \author[\instMPGHLL]{J.~Ninkovic,} % 2386
% \author[\instBNL]{N.~K.~Nisar,} % 2522
  \author[\instKEK,\instSOKENDAI,\instNiigata]{S.~Nishida,} % 2571
% \author[\instHawaii]{K.~Nishimura,} % 3063
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Novosel,} % 15523
% \author[\instNiigata]{K.~Ogawa,} % 2430
  \author[\instToho]{S.~Ogawa,} % 6263
% \author[\instCAU]{S.~L.~Olsen,} % 4563
  \author[\instKyiv]{Y.~Onishchuk,} % 2157
  \author[\instNiigata]{H.~Ono,} % 2160
% \author[\instUTokyo]{Y.~Onuki,} % 2331
% \author[\instIJCLab]{P.~Oskin,} % 9623
% \author[\instUTokyo]{F.~Otani,} % 16244
% \author[\instCMU]{E.~R.~Oxford,} % 6943
% \author[\instKEK,\instSOKENDAI]{H.~Ozaki,} % 2984
% \author[\instHSE]{P.~Pakhlov,} % 2221
  \author[\instHSE]{G.~Pakhlova,} % 2188
% \author[\instPisaUNIV,\instPisaINFN]{A.~Paladino,} % 2435
% \author[\instPittsburgh]{T.~Pang,} % 2114
% \author[\instMississippi]{A.~Panta,} % 7943
% \author[\instPisaUNIV,\instPisaINFN]{E.~Paoloni,} % 2488
  \author[\instNapoliINFN]{S.~Pardi,} % 2532
  \author[\instDuke]{K.~Parham,} % 10684
  \author[\instKyungpook]{H.~Park,} % 2284
  \author[\instUTokyo]{J.~Park,} % 18203
  \author[\instKEK]{S.-H.~Park,} % 2509
% \author[\instBonn]{B.~Paschen,} % 2159
  \author[\instRomaTreINFN]{A.~Passeri,} % 2116
  \author[\instLouisville]{S.~Patra,} % 3123
  \author[\instTUM]{S.~Paul,} % 2131
  \author[\instLuther]{T.~K.~Pedlar,} % 2421
% \author[\instFrascati]{I.~Peruzzi,} % 2253
  \author[\instHawaii]{R.~Peschke,} % 7123
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{R.~Pestotnik,} % 2476
% \author[\instMelbourne]{F.~Pham,} % 2963
  \author[\instFrascati]{M.~Piccolo,} % 2147
  \author[\instVPI]{L.~E.~Piilonen,} % 2346
  \author[\instTorinoUNIV,\instTorinoINFN]{G.~Pinna~Angioni,} % 13363
  \author[\instUAS]{P.~L.~M.~Podesta-Lerma,} % 2266
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{T.~Podobnik,} % 11223
  \author[\instMississippi]{S.~Pokharel,} % 12283
% \author[\instCPPM]{L.~Polat,} % 9783
% \author[\instTelAviv,\instHSE]{V.~Popov,} % 2096
  \author[\instKEK]{C.~Praz,} % 2726
  \author[\instISU]{S.~Prell,} % 12743
  \author[\instGiessen]{E.~Prencipe,} % 2219
  \author[\instBonn]{M.~T.~Prim,} % 2501
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{I.~Prudiiev,} % 19383
% \author[\instSCarolina]{M.~V.~Purohit,} % 2196
  \author[\instHawaii]{H.~Purwar,} % 12363
% \author[\instTUM]{A.~Rabusov,} % 2355
% \author[\instDESY]{N.~Rad,} % 11683
  \author[\instHEPHYVienna]{P.~Rados,} % 7383
  \author[\instHEPHYVienna]{G.~Raeuber,} % 18143
  \author[\instTriesteUNIV,\instTriesteINFN]{S.~Raiz,} % 13003
  \author[\instGoettingen]{N.~Rauls,} % 11603
% \author[\instTata]{K.~Ravindran,} % 22503
  \author[\instMPP]{M.~Reif,} % 8043
  \author[\instGiessen]{S.~Reiter,} % 2248
  \author[\instBINP,\instNSU]{M.~Remnev,} % 2785
  \author[\instKarlsruhe]{L.~Reuter,} % 16403
  \author[\instIPHC]{I.~Ripp-Baudot,} % 2469
% \author[\instHeidelberg]{M.~Ritzert,} % 2526
  \author[\instPisaUNIV,\instPisaINFN]{G.~Rizzo,} % 2579
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~B.~Rizzuto,} % 3746
% \author[\instUofA,\instIPP]{S.~H.~Robertson,} % 2471
% \author[\instMelbourne]{P.~Rocchetti,} % 13763
% \author[\instUAS]{D.~Rodr\'{i}guez~P\'{e}rez,} % 2176
  \author[\instDESY]{M.~Roehrken,} % 11883
  \author[\instVictoria,\instIPP]{J.~M.~Roney,} % 2244
% \author[\instSCarolina]{C.~Rosenfeld,} % 2082
  \author[\instDESY]{A.~Rostomyan,} % 2481
  \author[\instTriesteINFN]{N.~Rout,} % 2965
% \author[\instKrakow]{M.~Rozanska,} % 2205
% \author[\instNapoliUNIV,\instNapoliINFN]{G.~Russo,} % 2388
% \author[\instISU]{D.~Sahoo,} % 2110
% \author[\instKEK,\instSOKENDAI]{Y.~Sakai,} % 2175
% \author[\instMississippi]{D.~A.~Sanders,} % 2458
  \author[\instIITHyderabad]{S.~Sandilya,} % 2286
% \author[\instCincinnati]{A.~Sangal,} % 2384
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~Santelj,} % 2185
% \author[\instTohoku]{T.~Sanuki,} % 6783
% \author[\instPadovaUNIV,\instPadovaINFN]{P.~Sartori,} % 4523
  \author[\instKEK]{Y.~Sato,} % 5243
  \author[\instPittsburgh]{V.~Savinov,} % 2292
  \author[\instUppsala]{B.~Scavino,} % 2518
% \author[\instLMU,\instMPP]{C.~Schmitt,} % 15063
% \author[\instBonn]{J.~Schmitz,} % 12863
  \author[\instDuke]{S.~Schneider,} % 16803
% \author[\instBilbao,\instIKERBASQUE]{G.~Schnell,} % 12204
  \author[\instKarlsruhe]{M.~Schnepf,} % 15683
% \author[\instHawaii]{J.~Schueler,} % 2824
  \author[\instHEPHYVienna]{C.~Schwanda,} % 2108
% \author[\instCincinnati]{A.~J.~Schwartz,} % 2162
% \author[\instGoettingen]{B.~Schwenker,} % 2405
% \author[\instGoettingen]{M.~Schwickardi,} % 14743
% \author[\instRIKENBNL]{R.~Seidl,} % 26923
  \author[\instNiigata]{Y.~Seino,} % 2517
  \author[\instRomaTreINFN]{A.~Selce,} % 9043
  \author[\instYamagata]{K.~Senyo,} % 2987
  \author[\instCPPM]{J.~Serrano,} % 12124
  \author[\instMelbourne]{M.~E.~Sevior,} % 2328
  \author[\instMainz]{C.~Sfienti,} % 2214
  \author[\instHUNNU]{W.~Shan,} % 11943
% \author[\instIHEPRussia]{M.~Shapkin,} % 2460 
  \author[\instMNITJaipur]{C.~Sharma,} % 11584
% \author[\instHawaii]{V.~Shebalin,} % 2339
  \author[\instFudan]{C.~P.~Shen,} % 2464
  \author[\instKEK]{X.~D.~Shi,} % 18843
% \author[\instToho]{H.~Shibuya,} % 2234
  \author[\instMcGill]{T.~Shillington,} % 7983
  \author[\instUTokyo]{T.~Shimasaki,} % 16263
  \author[\instNTUTaiwan]{J.-G.~Shiu,} % 2412
  \author[\instBINP,\instNSU]{D.~Shtol,} % 9223
% \author[\instBINP,\instNSU]{B.~Shwartz,} % 2122
  \author[\instHawaii]{A.~Sibidanov,} % 2419
  \author[\instKarlsruhe]{F.~Simon,} % 2164
  \author[\instPanjab,\instUPES]{J.~B.~Singh,} % 2903
% \author[\instHawaii]{R.~Sinha,} % 3423
  \author[\instMPP,\instTUM]{J.~Skorupa,} % 12523
% \author[\instMelbourne]{K.~Smith,} % 2243
  \author[\instVictoria,\instIPP]{R.~J.~Sobie,} % 2472
  \author[\instMainz]{M.~Sobotzik,} % 8604
  \author[\instTelAviv]{A.~Soffer,} % 2217
% \author[\instIHEPRussia]{A.~Sokolov,} % 2521
% \author[\instDESY]{Y.~Soloviev,} % 2479
  \author[\instBINP]{E.~Solovieva,} % 2398
  \author[\instJLU]{W.~Song,} % 22863
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Spataro,} % 2117
  \author[\instMainz]{B.~Spruck,} % 2493
% \author[\instNovaGorica]{S.~Stani\v{c},} % 3383
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{M.~Stari\v{c},} % 2326
  \author[\instIPHC]{P.~Stavroulakis,} % 20643
  \author[\instKarlsruhe]{S.~Stefkova,} % 8783
% \author[\instVPI]{Z.~S.~Stottler,} % 2267
  \author[\instPadovaUNIV,\instPadovaINFN]{R.~Stroili,} % 2465
% \author[\instPNNL]{J.~Strube,} % 2451
% \author[\instNagoya]{Y.~Sue,} % 2085
% \author[\instUTokyo]{R.~Sugiura,} % 4644
  \author[\instRCNP,\instGifu]{M.~Sumihama,} % 4243
  \author[\instKEK,\instSOKENDAI,\instNaraWu]{K.~Sumisawa,} % 2583
% \author[\instBonn]{W.~Sutcliffe,} % 3784
  \author[\instChula]{N.~Suwonjandee,} % 14063
% \author[\instKEK,\instSOKENDAI]{S.~Y.~Suzuki,} % 2496
  \author[\instDESY]{H.~Svidras,} % 11783
% \author[\instChiba]{M.~Tabata,} % 2986
  \author[\instDESY]{M.~Takahashi,} % 2467
  \author[\instSPU,\instJPARC,\instRIKENMSL]{M.~Takizawa,} % 2437
% \author[\instTorinoINFN]{U.~Tamponi,} % 2366
  \author[\instKEK,\instSOKENDAI]{S.~Tanaka,} % 2530
  \author[\instJAEA]{K.~Tanida,} % 3803
% \author[\instUTokyo]{H.~Tanigawa,} % 2237
% \author[\instKEK]{N.~Taniguchi,} % 2285
  \author[\instPisaUNIV,\instPisaINFN]{F.~Tenchini,} % 2546
% \author[\instOsakaMetropolitan]{Y.~Teramoto,} % 26063
  \author[\instCPPM]{A.~Thaller,} % 16044
  \author[\instMPP]{O.~Tittel,} % 8663
  \author[\instTata]{R.~Tiwary,} % 10403
  \author[\instTriesteINFN]{D.~Tonelli,} % 4564
  \author[\instPadovaINFN]{E.~Torassa,} % 2556
% \author[\instSydney]{N.~Toutounji,} % 2263
  \author[\instTYL]{K.~Trabelsi,} % 2369
% \author[\instBonn]{I.~Tsaklidis,} % 13443
% \author[\instKEK,\instSOKENDAI]{T.~Tsuboyama,} % 2361
% \author[\instNagoya]{N.~Tsuzuki,} % 2352
% \author[\instTitech]{M.~Uchida,} % 2370
  \author[\instKEK,\instSOKENDAI]{I.~Ueda,} % 2519
% \author[\instKEK,\instSOKENDAI]{S.~Uehara,} % 2586
% \author[\instUTokyo]{Y.~Uematsu,} % 5883
  \author[\instHSE]{T.~Uglov,} % 2252
  \author[\instKarlsruhe]{K.~Unger,} % 9463
  \author[\instHanyang]{Y.~Unno,} % 2420
  \author[\instKEK]{K.~Uno,} % 14963
  \author[\instKEK,\instSOKENDAI]{S.~Uno,} % 2149
% \author[\instMelbourne]{P.~Urquijo,} % 2302
% \author[\instKEK,\instUTokyo,\instSOKENDAI]{Y.~Ushiroda,} % 2317
% \author[\instBINP,\instNSU]{Y.~V.~Usov,} % 5003
  \author[\instHawaii]{S.~E.~Vahsen,} % 2251
  \author[\instMcGill]{R.~van~Tonder,} % 2706
% \author[\instHawaii]{G.~S.~Varner,} % 2119
  \author[\instSydney]{K.~E.~Varvell,} % 2545
  \author[\instISU]{M.~Veronesi,} % 20723
  \author[\instBINP,\instNSU]{A.~Vinokurova,} % 2289
  \author[\instIITHyderabad]{V.~S.~Vismaya,} % 16063
  \author[\instTriesteUNIV,\instTriesteINFN]{L.~Vitale,} % 2415
  \author[\instIJCLab]{V.~Vobbilisetti,} % 7364
  \author[\instPerugiaUNIV,\instPerugiaINFN]{R.~Volpe,} % 20183
% \author[\instBINP]{V.~Vorobyev,} % 2298
  \author[\instDuke]{A.~Vossen,} % 2249
% \author[\instMPP,\instTUM]{B.~Wach,} % 8203
% \author[\instKEK]{E.~Waheed,} % 2226
  \author[\instUBC]{M.~Wakai,} % 3583
% \author[\instMcGill]{H.~M.~Wakeling,} % 3664
  \author[\instMPP]{S.~Wallner,} % 20363
% \author[\instMalaya]{W.~Wan~Abdullah,} % 2280
% \author[\instMPP]{B.~Wang,} % 2569
% \author[\instNUUTaiwan]{C.~H.~Wang,} % 2224
  \author[\instPittsburgh]{E.~Wang,} % 10983
  \author[\instNTUTaiwan]{M.-Z.~Wang,} % 2074
% \author[\instFudan]{X.~L.~Wang,} % 2076
  \author[\instUTokyo]{Z.~Wang,} % 15743
  \author[\instMcGill]{A.~Warburton,} % 2347
% \author[\instNiigata]{M.~Watanabe,} % 2309
  \author[\instCincinnati]{S.~Watanuki,} % 6843
% \author[\instBonn]{M.~Welsch,} % 7023
% \author[\instTriesteINFN]{O.~Werbycka,} % 6123
  \author[\instDESY]{C.~Wessel,} % 2100
% \author[\instKrakow]{J.~Wiechczynski,} % 2604
% \author[\instGoettingen]{P.~Wieduwilt,} % 2343
% \author[\instMPP]{H.~Windel,} % 2081
  \author[\instKoreaUnivKU]{E.~Won,} % 2410
% \author[\instShandong]{Y.~Xie,} % 20383
  \author[\instSoochow]{X.~P.~Xu,} % 4923
  \author[\instSydney]{B.~D.~Yabsley,} % 3645
  \author[\instKEK]{S.~Yamada,} % 2492
% \author[\instTohoku]{H.~Yamamoto,} % 2964
  \author[\instUSTC]{W.~Yan,} % 2094
  \author[\instKoreaUnivKU]{S.~B.~Yang,} % 2374
  \author[\instFlorida]{J.~Yelton,} % 2067
  \author[\instNankai]{J.~H.~Yin,} % 2365
  \author[\instIHEPChina]{Y.~M.~Yook,} % 2453
  \author[\instHawaii]{K.~Yoshihara,} % 12663
  \author[\instIHEPChina]{C.~Z.~Yuan,} % 2088
% \author[\instNiigata]{Y.~Yusa,} % 2357
  \author[\instRomaTreUNIV,\instRomaTreINFN]{L.~Zani,} % 2529
  \author[\instIPMU]{F.~Zeng,} % 22043
  \author[\instHawaii]{B.~Zhang,} % 11663
% \author[\instIHEPChina]{J.~Z.~Zhang,} % 2349
% \author[\instFudan]{Y.~Zhang,} % 3303
% \author[\instUSTC]{Z.~Zhang,} % 5363
  \author[\instBINP,\instNSU]{V.~Zhilich,} % 4703
  \author[\instFudan]{J.~S.~Zhou,} % 12463
  \author[\instShandong]{Q.~D.~Zhou,} % 7323
% \author[\instLNNU]{X.~Y.~Zhou,} % 2380
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{V.~I.~Zhukova,} % 2387
% \author[\instBINP,\instNSU]{V.~Zhulanov,} % 4983
  \author[\instPrague]{R.~\v{Z}leb\v{c}\'{i}k} % 13403
%%%\affiliation[\instKAU]{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589, Saudi Arabia}
\affiliation[\instCPPM]{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\affiliation[\instYerevan]{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\affiliation[\instGoettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
%%%\affiliation[\instBeihang]{Beihang University, Beijing 100191, China}
\affiliation[\instBNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\affiliation[\instBINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
%%%\affiliation[\instCMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\affiliation[\instCinvestavIPN]{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\affiliation[\instPrague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\affiliation[\instChiangMai]{Chiang Mai University, Chiang Mai 50202, Thailand}
%%%\affiliation[\instChiba]{Chiba University, Chiba 263-8522, Japan}
\affiliation[\instChonnam]{Chonnam National University, Gwangju 61186, South Korea}
\affiliation[\instChula]{Chulalongkorn University, Bangkok 10330, Thailand}
\affiliation[\instCAU]{Chung-Ang University, Seoul 06974, South Korea}
\affiliation[\instConacyt]{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\affiliation[\instDESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\affiliation[\instDuke]{Duke University, Durham, North Carolina 27708, U.S.A.}
\affiliation[\instITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\affiliation[\instFuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\affiliation[\instFudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\affiliation[\instGifu]{Gifu University, Gifu 501-1193, Japan}
\affiliation[\instSOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\affiliation[\instMainz]{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\affiliation[\instGyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\affiliation[\instHanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
%%%\affiliation[\instHeidelberg]{Heidelberg University, 68131 Mannheim, Germany}
%%%\affiliation[\instHNU]{Henan Normal University, Xinxiang 453007, China}
\affiliation[\instKEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instJPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instHiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\affiliation[\instHUNNU]{Hunan Normal University, Changsha 410081, China}
%%%\affiliation[\instIKERBASQUE]{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao, Spain}
\affiliation[\instFrascati]{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\affiliation[\instNapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[\instPadovaINFN]{INFN Sezione di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaINFN]{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIISc]{Indian Institute of Science, Bengaluru 560012, India}
%%%\affiliation[\instIISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\affiliation[\instIITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\affiliation[\instIITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\affiliation[\instIITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
%%%\affiliation[\instIITJodhpur]{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\affiliation[\instIITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\affiliation[\instIndiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
%%%\affiliation[\instIHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\affiliation[\instHEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\affiliation[\instIHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affiliation[\instIPP]{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\affiliation[\instIOP]{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\affiliation[\instIFIC]{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\affiliation[\instISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\affiliation[\instJAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\affiliation[\instJLU]{Jilin University, Changchun 130012, China}
\affiliation[\instKarlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
%%%\affiliation[\instKitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\affiliation[\instKISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\affiliation[\instKoreaUnivKU]{Korea University, Seoul 02841, South Korea}
\affiliation[\instKSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\affiliation[\instKyotoU]{Kyoto University, Kyoto 606-8501, Japan}
\affiliation[\instKyungpook]{Kyungpook National University, Daegu 41566, South Korea}
%%%\affiliation[\instLNNU]{Liaoning Normal University, Dalian 116029, China}
\affiliation[\instGiessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\affiliation[\instLuther]{Luther College, Decorah, Iowa 52101, U.S.A.}
\affiliation[\instMNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\affiliation[\instLMU]{Ludwig Maximilians University, 80539 Munich, Germany}
\affiliation[\instMcGill]{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
%%%\affiliation[\instMETU]{Middle East Technical University, 06531 Ankara, Turkey}
%%%\affiliation[\instMEPhI]{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\affiliation[\instNagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\affiliation[\instNNU]{Nanjing Normal University, Nanjing 210023, China}
\affiliation[\instNankai]{Nankai University, Tianjin 300071, China}
\affiliation[\instNaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\affiliation[\instUNAM]{National Autonomous University of Mexico, Mexico City, Mexico}
\affiliation[\instHSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\affiliation[\instNTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
%%%\affiliation[\instNUUTaiwan]{National United University, Miao Li 36003, Taiwan}
\affiliation[\instKrakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\affiliation[\instNiigata]{Niigata University, Niigata 950-2181, Japan}
\affiliation[\instNSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\affiliation[\instOsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\affiliation[\instRCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\affiliation[\instPNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\affiliation[\instPanjab]{Panjab University, Chandigarh 160014, India}
\affiliation[\instMPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
%%%\affiliation[\instMPGHLL]{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\affiliation[\instPanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
%%%\affiliation[\instRIKENBNL]{RIKEN BNL Research Center, Upton, New York 11973, U.S.A.}
\affiliation[\instRIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\affiliation[\instSeoul]{Seoul National University, Seoul 08826, South Korea}
\affiliation[\instShandong]{Shandong University, Jinan 250100, China}
\affiliation[\instKyiv]{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\affiliation[\instSPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\affiliation[\instSoochow]{Soochow University, Suzhou 215006, China}
\affiliation[\instSoongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\affiliation[\instSEU]{Southeast University, Nanjing 211189, China}
\affiliation[\instLjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\affiliation[\instSKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
\affiliation[\instTata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\affiliation[\instTUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\affiliation[\instTelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\affiliation[\instToho]{Toho University, Funabashi 274-8510, Japan}
%%%\affiliation[\instTohoku]{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
%%%\affiliation[\instTitech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
%%%\affiliation[\instTokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\affiliation[\instUAS]{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\affiliation[\instNapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\affiliation[\instPadovaUNIV]{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaUNIV]{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoUNIV]{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteUNIV]{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[\instIPHC]{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\affiliation[\instAdelaide]{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
%%%\affiliation[\instUofA]{University of Alberta, Edmonton, Alberta, T6G 2E1, Canada}
%%%\affiliation[\instBilbao]{Department of Physics and EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao, Spain}
\affiliation[\instBonn]{University of Bonn, 53115 Bonn, Germany}
\affiliation[\instUBC]{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\affiliation[\instCincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\affiliation[\instFlorida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
\affiliation[\instHamburg]{University of Hamburg, 20148 Hamburg, Germany}
\affiliation[\instHawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\affiliation[\instLjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\affiliation[\instLouisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\affiliation[\instMalaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\affiliation[\instManitoba]{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\affiliation[\instLjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\affiliation[\instMelbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\affiliation[\instMississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
%%%\affiliation[\instUOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\affiliation[\instNovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\affiliation[\instUPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
\affiliation[\instPittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\affiliation[\instUSTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\affiliation[\instSAlabama]{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
%%%\affiliation[\instSCarolina]{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\affiliation[\instSydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
\affiliation[\instTabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\affiliation[\instUTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\affiliation[\instEri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\affiliation[\instIPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\affiliation[\instVictoria]{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\affiliation[\instUppsala]{Uppsala University, SE-751 05 Uppsala, Sweden}
\affiliation[\instVPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\affiliation[\instWayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
%%%\affiliation[\instXavier]{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\affiliation[\instXJTU]{Xi'an Jiaotong University, Xi'an 710049, China}
\affiliation[\instYamagata]{Yamagata University, Yamagata 990-8560, Japan}
\affiliation[\instYonsei]{Yonsei University, Seoul 03722, South Korea}
\affiliation[\instTYL]{Toshiko Yuasa Laboratory, Tsukuba 305-0801, Japan}
%%%\affiliation[\instZZU]{Zhengzhou University, Zhengzhou 450001, China}

